Cognitive biases can move opinion dynamics from consensus to signatures of transient chaos

Interest in how democracies form consensus has increased recently, with statistical physics and economics approaches both suggesting that there is convergence to a fixed point in belief networks, but with fluctuations in opinions when there are ``stubborn'' voters. We modify a model of opinion dynamics in which agents are fully Bayesian to account for two cognitive biases: confirmation bias and in-group bias. Confirmation bias occurs when the received information is considered to be more likely when it aligns with the receiver's beliefs. In-group bias occurs when the receiver further considers the information to be more likely when the receiver's beliefs and the sender's beliefs are aligned. We find that when there are no cognitive biases, a network of agents always converges to complete consensus. With confirmation bias alone, polarization can occur. With both biases present, consensus and polarization are possible, but when agents attempt to counteract confirmation bias, there can be signatures of transient chaos and ongoing opinion fluctuations. Based on this simple model, we conjecture that complex opinion fluctuations might be a generic feature of opinion dynamics when agents are Bayesian with biases.

==> cmechabbrev.tex <==
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}  {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\SampleSpace} { \AllPasts }
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\MeasSymbols}[2]{ \MeasSymbol_{#1:#2} }
\newcommand{\meassymbols}[2] { \meassymbol_{#1:#2} }
\newcommand{\BiInfinity}    { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}    { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past} { \smash{\overleftarrow {\MeasSymbol}} }
%\newcommand{\Past} { \MeasSymbols{}{0} }
\newcommand{\past} { {\smash{\overleftarrow {\meassymbol}}} }
%\newcommand{\past} { \meassymbols{}{0} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}   { \smash{\overrightarrow{\MeasSymbol}} }
%\newcommand{\Future} { \MeasSymbols{0}{} }
\newcommand{\future}   { \smash{\overrightarrow{\meassymbol}} }
%\newcommand{\future} { \meassymbols{0}{} }
\newcommand{\futureprime}   { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}   { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}  { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL} { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL} { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}    { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}  { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}    { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }
\newcommand{\rep}    { r }
\newcommand{\Rep}    { \mathcal{R} }
\newcommand{\repa}    { \widehat{r} }
\newcommand{\Repa}    { \widehat{\mathcal{R}} }
\newcommand{\repb}    { \widetilde{r} }
\newcommand{\Repb}    { \widetilde{\mathcal{R}} }


\newcommand{\Present} {\MeasSymbol_0}

% Causal states and epsilon-machines
\newcommand{\CausalState}   { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}   { \sigma }
\newcommand{\CausalStateSet}    { \bm{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}   { \AlternateState^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}   { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \bm{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \bm{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}  { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}  { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}     { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}       {C_\mu}
\newcommand{\hmu}       {h_\mu}
\newcommand{\EE}        {{\bf E}}
\newcommand{\TI}        {{\bf T}}
\newcommand{\SI}        {{\bf S}}
\newcommand{\SE}        { H_{\mathrm{sync}} }
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}        {\chi}

% Causal Irreversibility
\newcommand{\CI}        {\Xi}
\newcommand{\ReverseMap}    {r}
\newcommand{\ForwardMap}    {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\mathbf{\EstCausalState}}
\newcommand{\EstCausalFunc} {\widehat{\epsilon}}
\newcommand{\EstCmu}        {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}    { \mathcal{A}}
\newcommand{\insymbol}      { a}
\newcommand{\OutAlphabet}   { \mathcal{B}}
\newcommand{\outsymbol}     { b}
\newcommand{\InputSimple}   { X}
\newcommand{\inputsimple}   { x}
\newcommand{\BottleneckVar} {\tilde{\InputSimple}}
\newcommand{\bottleneckvar} {\tilde{\inputsimple}}
\newcommand{\InputSpace}    { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}   { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}   { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}    { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}  { Y}
\newcommand{\outputsimple}  { y}
\newcommand{\OutputSpace}   { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}    { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}    { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}  { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}  { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne} { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone} { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}    {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}    {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}   {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}    {{\InputPast}^{L}}
\newcommand{\inputpastL}    {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}  {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}  {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts} { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \mathbf{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}  { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}  { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}   { \mathcal{F}}
\newcommand{\feedbackcausalstate}   { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}      { \mathcal{J}}
\newcommand{\JointCausalStateSet}   { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}   { {\Omega}}
\newcommand{\naturestate}   { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}   { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}   {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}           { {\widehat{\Prob}_N}}
\newcommand{\STRegion}          { {\mathrm K}}
\newcommand{\STRegionVariable}      { K}
\newcommand{\stregionvariable}      { k}
\newcommand{\GlobalPast}        { \overleftarrow{G}}
\newcommand{\globalpast}        { \overleftarrow{g}}
\newcommand{\GlobalFuture}      { \overrightarrow{G}}
\newcommand{\globalfuture}      { \overrightarrow{g}}
\newcommand{\GlobalState}       { \mathcal{G}}
\newcommand{\globalstate}       { \gamma}
\newcommand{\GlobalStateSet}        { {\mathbf \GlobalState}}
\newcommand{\LocalPast}         { \overleftarrow{L}}
\newcommand{\localpast}         { \overleftarrow{l}}
\newcommand{\AllLocalPasts}     { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}       { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}       { \overrightarrow{L}}
\newcommand{\localfuture}       { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}     { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}        { \mathcal{L}}
\newcommand{\localstate}        { \lambda}
\newcommand{\LocalStateSet}     { {\mathbf \LocalState}}
\newcommand{\PatchPast}         { \overleftarrow{P}}
\newcommand{\patchpast}         { \overleftarrow{p}}
\newcommand{\PatchPastRegion}       { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}       { \overrightarrow{P}}
\newcommand{\patchfuture}       { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}     { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}        { \mathcal{P}}
\newcommand{\patchstate}        { \pi}
\newcommand{\PatchStateSet}     { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}    {\vec{\LocalState}}
\newcommand{\localstatesinpatch}    {\vec{\localstate}}
\newcommand{\PointInstantX}     { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}         { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}    {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]    { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]    { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]      { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]      { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}  { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess} { {\Process}^{\forward} }
\newcommand{\PastProcess}   { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}  { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}     { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}     { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}  { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}    { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}      { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}     { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps} { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}        {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}    { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}    { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2},\CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbols{#1}{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbols{#1}{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbols{#1}{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbols{#1}{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbols{#1}{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\SGBE}[2][0]{
  \ensuremath{H[\CausalState_{#2} | \MeasSymbols{#1}{#2}]}
}

\newcommand{\GI}{\varphi}
\newcommand{\OI}{\zeta}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{k_{\PC}}
\newcommand{\GOrder}{k_{\GI}}
\newcommand{\OOrder}{k_{\OI}}
\newcommand{\MOrder}{R}
\newcommand{\SOrder}{k_{\SI}}
\newcommand{\Lsync} {\mathcal{L}_{\mathrm{sync}}}

%% stuff for the anatomy paper

\newcommand{\rhomu}{\rho_\mu}
\newcommand{\rmu}{r_\mu}
\newcommand{\bmu}{b_\mu}
\newcommand{\qmu}{q_\mu}
\newcommand{\wmu}{w_\mu}
\newcommand{\imu}{i_\mu}
\newcommand{\sigmamu}{\sigma_\mu}
\newcommand{\EER}{\EE_R}
\newcommand{\EEB}{\EE_B}
\newcommand{\EEQ}{\EE_Q}
\newcommand{\EEW}{\EE_W}
\newcommand{\I}{\mathbf{I}}

%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}

%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi




